What determines large scale galaxy clustering: halo mass or local density?

Using dark matter simulations we show how halo bias is determined by local density and not by halo mass. This is not totally surprising, as according to the peak-background split model, local density is the property that constraints bias at large scales. Massive haloes have a high clustering because they reside in high density regions. Small haloes can be found in a wide range of environments which determine their clustering amplitudes differently. This contradicts the assumption of standard Halo Occupation Distribution (HOD) models that the bias and occupation of haloes is determined solely by their mass. We show that the bias of central galaxies from semi-analytic models of galaxy formation as a function of luminosity and colour is not correctly predicted by the standard HOD model. Using local density instead of halo mass the HOD model correctly predicts galaxy bias. These results indicate the need to include information about local density and not only mass in order to correctly apply HOD analysis in these galaxy samples. This new model can be readily applied to observations and has the advantage that the galaxy density can be directly observed, in contrast with the dark matter halo mass.

==> sections/intro.tex <==

\section{Introduction}
In the standard cosmological framework, the so-called ${\Lambda}$CDM
paradigm, galaxies form, evolve and reside in dark matter haloes that
grow and assemble in a hierarchical way \citep{White1978}.
Therefore, the evolution and the properties of the host haloes will
have a strong impact in determining the galaxy properties themselves. \noelia{ change this-The
unknown nature of the dark matter (and dark energy) can be unveiled
through the study of the baryonic observables (such as galaxies) once we model
the co-evolution with their host dark matter haloes}. Modelling the relation between the observed galaxy distribution and the underlying dark matter field is a fundamental problem in modern cosmology.
 
Given a cosmology, the halo mass function, the halo concentration, and the halo bias can be defined.
In order to model the galaxy clustering statistics it is necessary to specify the
number and spatial distribution of galaxies within the dark matter
haloes. The probability that a halo of mass $M$ hosts
$N_{gal}$ galaxies of a given property is
given by the quantity $P(N_{gal}|M)$. This statistical halo distribution is known as the 'Halo Occupation Distribution'
  \citep[hereafter referred to as HOD,][]{Jing1998,Benson2000,Seljak2000,Scoccimarro2001,Cooray2002,Berlind2002}.
  Therefore, its simplicity resides in the assumption  that the derived parameters for the cosmological model  and the physical properties of the galaxies are determined solely by
  the mass of the halo in which they reside.

 \noelia{ add this -- point out more in the intro that the we expect the number of galaxies per halo,
(which is the main HOD prediction I guess) to be wrong, when the bias prediction fails.
Explicitly: if the HOD model in eq five is wrong then
- N(m,P) will be wrong for for a given b(P) (that?s what happens when you vary N in order to match an observed bias b) or - b(P) will be wrong for a given N(m,P) (that?s our test).

 the key concept that underlies halo occupation modeling is that all galaxies reside in dark matter halos, and that these halos themselves are biased tracers of the dark matter density field. If the so-called halo bias" bh were only a function of halo mass, then knowledge of the manner by which galaxies reside in halos as a function of halo mass would be suficcient to make predictions for the
large-scale galaxy clustering that we observe. In its standard form, HOD modeling assumes that the galaxy content of a halo of fixed mass is independent of the halo?s large scale environment.
To the extent that this assumption holds, the HOD allows a complete description of the relation
between galaxies and mass, from large scales into the fully non-linear regime.}
Conventional HOD formulations assume that only halo mass governs the galaxy-halo connection. Violations of this assumption, known as galaxy assembly bias, threaten the HOD program. }


The HOD has been proven to be a very powerful theoretical tool to constrain
both the galaxy-halo connection and the fundamental parameters in
cosmology \citep{Yang2003,Zehavi2005,Cooray2006,vdBosch2007,Zheng2007,Zehavi2011,Tinker2013}. 
By the use of the HOD model mock galaxy
catalogues are constructed for studies of  galaxy formation as well as for the preparation and analysis of  observational surveys \citep{Berlind2002,Zheng2007, BOSS2015,Carretero2015}.
 However, it has become clear that the clustering of dark
matter haloes depends on other properties besides mass \citep{Sheth2004,Gao2005,Wechsler2006,Gao2007,Jing2007,Wetzel2007, Falta2010,Lacerna2011,Lacerna2014}.


 The construction of mock galaxy catalogues through N-body simulations has
 shown that the amplitude of the two-point correlation function of
 dark matter haloes with masses lower than $10^{13}\Mo$ on large scales
 depends on halo formation time \citep[e.g.,][]{Gao2005}.  Additionally, 
 halo properties such as concentration, shape, halo spin, major merger rate, triaxiality, shape of the velocity ellipsoid and velocity anisotropy  show correlations with other properties than  halo mass  \citep{Bett2007,Croton2007,Lacerna2012}.
 Moreover, haloes of equal mass could have different galaxy occupation statistics, depending on their  environment \citep[e.g.,][]{Croft2012,Pujol2014}. Ignoring the effects of
 properties other than mass in the HOD modelling could distort the
 conclusions and interpretations of the observational results
 \citep{Zentner2014}.

Several studies point in the direction of taking into account halo properties linked with the environment and their formation history to modify the standard HOD. This is sometimes called assembly bias. These properties are incorporated in the formulation of more flexible schemes of HOD used to produce mock catalogues comparable with observations. 
 Such mock catalogues have recently been presented by 
\cite{Croton2007} and \cite{Masaki2013}, who introduced a rank ordering of galaxy
colours or Star Formation Rate (SFR). They found that for fixed halo mass, red galaxies are more clustered than blue galaxies. These and the 'age matching' models of \citet{Hearin2013,Hearin2014} have been shown to successfully reproduce
a number of observed signals such as the two-point clustering and
galaxy-galaxy lensing signal of SDSS galaxies (\citealt{Lacerna2014} and references therein).

%In this work, we aim to study the dependence of halo bias on mass and environment from the HOD paradigm,
%by studying how well mass and environment 
%determine the galaxy bias and recovers the clustering in terms of
%different galaxy properties in a self consistent way.  We study the
%halo bias using the Peak Background Split model {hereafter referred to as PBS}
%\citep{Bardeen1986,ColeKaiser1989}.
%In the PSB calculations the fundamental quantity is the density of the dark matter field
%${\bar \delta}$ and not $M$. This motivates our choice for the study.

In this work we study the dependence of large scale halo bias on mass and \arnau{local density}, in order to analyse how well mass and \arnau{density} allow to correctly determine galaxy bias. 
Our analysis is based on haloes from the Millennium simulation \citep{Springel2005} \arnau{and the Semi-Analytical Model} (SAM) of galaxy formation of \citet{Guo2011}. The SAM  populate  haloes with galaxies that are evolved and followed in time
inside the complex structure of merger-trees. The baryonic processes
included are laws for metal dependent gas cooling, reionization, star
formation, gas accretion, merging, disk instabilities, AGN and
supernovae feedback, ram pressure stripping and dust extinction, among others
\citep[e.g.,][]{Baugh2006,Jimenez11,Gargiulo2015}.  Because of these processes, the
resulting galaxy population produced by SAMs is sensitive to the environment and evolution of haloes. Depending on the galaxy selection, the information from halo mass alone could be insufficiently correlated with the clustering of galaxies. In these cases, \arnau{local} density allows to determine galaxy bias better than halo mass. Thus, we propose to use the information from local density to improve the HOD analyses on surveys and theory. 

The method employed in our study is similar to the one used in \citet{Pujol2014} which performs a direct HOD reconstruction instead of a HOD fit. We compare the measured halo and galaxy bias with a HOD reconstruction based on direct measurements of the halo occupation, so there is not assumptions or fitting involved. Then, these predictions can be compared with the true bias in the simulation.

The paper is organized as follows. In section \ref{sec:methodology}
we describe the data used and the methodology for our measurements of clustering, bias
and for our HOD reconstructions. The results are shown
in section \ref{sec:results}, and we summarize the conclusions of the
paper in section \ref{sec:conclusions}.

 

==> sections/simulation.tex <==
\section{simulation data}\label{sec:simulation}


In this study we use the data from Millennium Simulation \footnote{\url{http://www.mpa-garching.mpg.de/millennium/}} \citep{Springel2005}, an N-body simulation generated using the \textsc{GADGET-2} code \citep{Springel2005b}. The simulation corresponds to a $\Lambda$-CDM cosmology with the following parameters: $\Omega_m = 0.25$, $\Omega_b = 0.045$, $h = 0.73$,  $\Omega_\Lambda = 0.75$, $n = 1$ and $\sigma_8 = 0.9$. It contains $2160^3$ particles in a comoving box of $500\Mpc$ of size. The resolution corresponds to a particle mass of $8.6 \times 10^8 \Mo$ and a spatial resolution of $5\kpc$. \arnau{The cosmological model is based on WMAP-1 \citep{Spergel2003} the 2-Degree Fields Galaxy Redshift Survey (2dFGRS) data \citep{Cole2005}. The initial conditions have been calculated using CMBFAST \citep{Seljak1996}. }
We use a comoving output at $z=0$.

The haloes are identified using the Friends-of-Friends (FOF) algorithm, using a linking length of $0.2$ times the mean particle separation, and discarding all the haloes with less than $20$ particles. Once the FOFs are identified, the \textsc{SUBFIND} algorithm \citep{Springel2001} has been applied to define subhaloes inside the haloes. Again, all subhaloes with fewer than $20$ particles have been discarded. In our analysis we define the halo mass from the total number of particles belonging to the FOFs, and the subhalo mass from the total number of particles belonging to the \textsc{SUBFIND} objects. 

\arnau{we can play a bit with the virial mass too}
